Multivariate Wasserstein Functional Connectivity for Autism Screening

Most approaches to the estimation of brain functional connectivity from the functional magnetic resonance imaging (fMRI) data rely on computing some measure of statistical dependence, or more generally, a distance between univariate representative time series of regions of interest (ROIs) consisting of multiple voxels. However, summarizing a ROI's multiple time series with its mean or the first principal component (1PC) may result to the loss of information as, for example, 1PC explains only a small fraction of variance of the multivariate signal of the neuronal activity. We propose to compare ROIs directly, without the use of representative time series, defining a new measure of multivariate connectivity between ROIs, not necessarily consisting of the same number of voxels, based on the Wasserstein distance. We assess the proposed Wasserstein functional connectivity measure on the autism screening task, demonstrating its superiority over commonly used univariate and multivariate functional connectivity measures.

==> figures/figure2.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=8.25cm]{figures/images/figure2.png}
\caption{\textbf{Left:} Pearson correlation connectivity matrix. \textbf{Right:} Wasserstein distance connectivity matrix.}
\label{figures:figure2}
%\vspace{-0.75em}
\end{figure}

==> figures/figure2_3.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=8.615cm]{figures/images/figure2.png}
\vspace{-1.5em}
\caption{Mean connectivity matrices. \textbf{Left:} Pearson correlation. \textbf{Center:} Distance correlation. \textbf{Right:} Wasserstein distance.}
\label{figures:figure2}
\vspace{-1em}
\end{figure}

==> figures/figure3.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{figures/images/figure3.png}
\caption{\textbf{Left:} Pearson correlation connectivity matrix. \textbf{Right:} Wasserstein distance connectivity matrix.}
\label{figures:figure2}
%\vspace{-0.75em}
\end{figure*}

==> figures/figure_all.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/CALTECH_116.png}
\includegraphics[width=17.5cm]{figures/images/KKI_116.png}
\includegraphics[width=17.5cm]{figures/images/LEUVEN_1_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/LEUVEN_2_116.png}
\includegraphics[width=17.5cm]{figures/images/LEUVEN_116.png}
\includegraphics[width=17.5cm]{figures/images/MAX_MUN_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/NYU_116.png}
\includegraphics[width=17.5cm]{figures/images/OHSU_116.png}
\includegraphics[width=17.5cm]{figures/images/OLIN_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/PITT_116.png}
\includegraphics[width=17.5cm]{figures/images/SDSU_116.png}
\includegraphics[width=17.5cm]{figures/images/STANFORD_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/TRINITY_116.png}
\includegraphics[width=17.5cm]{figures/images/UCLA_1_116.png}
\includegraphics[width=17.5cm]{figures/images/UCLA_2_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/UCLA_116.png}
\includegraphics[width=17.5cm]{figures/images/UM_1_116.png}
\includegraphics[width=17.5cm]{figures/images/UM_2_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=17.5cm]{figures/images/UM_116.png}
\includegraphics[width=17.5cm]{figures/images/USM_116.png}
\includegraphics[width=17.5cm]{figures/images/YALE_116.png}
%\caption{\small Classification results.}
%\label{figures:figure1}
\vspace{-0.75em}
\end{figure*}



==> sections/_figures.tex <==
\input{figures/figure1}

==> sections/_tables.tex <==
\newpage
%\section{Tables}
\input{tables/table1}
\input{tables/table2}

==> tables/table1.tex <==


\begin{table*}[h]
\centering
\begin{tabular}{|p{3cm}p{2cm}p{1cm}|lll|} \hline
Age group & Site        & Size    &Pearson r     & Wasserstein r & $\mathrm{\Delta}$ \\ \hline \hline
\multirow{16}{*}{All age groups}
& Caltech  & 37      & 60.6          & \textbf{65.0} & +4.4 \\
& KKI      & 39      & 61.1          & \textbf{69.2} & +8.1 \\
& Leuven   & 61      & 56.3          & \textbf{58.8} & +2.5 \\
& MaxMun   & 42      & 55.9          & \textbf{61.3} & +5.4 \\
& NYU      & 171     & \textbf{67.5} & 62.9          & -4.6 \\
& OHSU     & 23      & 61.7          & \textbf{64.0} & +2.3 \\
& Olin     & 25      & 66.7          & \textbf{68.5} & +0.8 \\
& Pitt     & 45      & 66.2          & \textbf{71.7} & +5.5 \\
& SBL      & 26      & \textbf{65.3} & 63.0          & -2.3 \\
& SDSU     & 33      & 53.7          & \textbf{60.5} & +6.8 \\
& Stanford & 36      & 60.5          & \textbf{85.3} & +24.8 \\
& Trinity  & 44      & \textbf{55.7} & 55.3          & -0.4 \\
& UCLA     & 75      & \textbf{68.9} & 67.5          & -1.4 \\
& UM       & 113     & 65.4          & \textbf{70.7} & +5.3 \\
& USM      & 61      & \textbf{67.6} & 61.8          & -5.8 \\ 
& Yale     & 48      & \textbf{73.1} & 61.3          & -11.8 \\ \hline \hline
\multirow{16}{*}{Best age group}
& Caltech  & 37      & \textbf{67.2} & 64.1          & -3.1 \\
& KKI      & 39      & 61.1          & \textbf{69.2} & +8.1 \\
& Leuven   & 61      & 63.5          & \textbf{65.7} & +2.2 \\
& MaxMun   & 42      & 47.7          & \textbf{62.1} & +14.4 \\
& NYU      & 171     & \textbf{68.2} & 68.0          & -0.2 \\
& OHSU     & 23      & \textbf{54.3} & 53.7          & -0.6 \\
& Olin     & 25      & \textbf{66.6} & 51.6          & -15.0 \\
& Pitt     & 45      & 62.5          & \textbf{87.5} & +25.0 \\
& SBL      & 26      & \textbf{65.3} & 63.0          & -2.3 \\
& SDSU     & 33      & 55.0          & \textbf{79.2} & +24.2 \\
& Stanford & 36      & 60.5          & \textbf{85.3} & +24.8 \\
& Trinity  & 44      & 54.9          & 50.6          & -4.3 \\
& UCLA     & 75      & \textbf{67.7} & 61.2          & -6.5 \\
& UM       & 113     & 60.2          & \textbf{70.2} & +10.0 \\
& USM      & 61      & \textbf{74.0} & 53.5          & -20.5 \\ 
& Yale     & 48      & 67.0          & \textbf{79.7} & +22.7 \\ \hline
\end{tabular}
\vspace{0.4em}
\caption{Wasserstein functional connectivity, ABIDE1 dataset.}
\label{table:results}
\end{table*}

==> tables/table1_parcellations.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{2.5cm}lll|}
\hline
                               & \multicolumn{1}{c}{Pearson} & \multicolumn{2}{c|}{Wasserstein connectivity}                 \\
                               & \multicolumn{1}{c}{r}       & \multicolumn{1}{c}{$W_1$} & \multicolumn{1}{c|}{$W_2$} \\ \hline \hline
\multicolumn{1}{|l|}{AAL}      &~\textbf{59.2$\pm$0.0}           &~55.4$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{BASC}   &~60.3$\pm$0.0                    &~\textbf{61.9$\pm$0.0}      &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{MSDL}   &~61.1$\pm$0.0                    &~\textbf{64.3$\pm$0.0}      &~00.0$\pm$0.0~                \\ \hline
\end{tabular}
\caption{Wasserstein functional connectivity. Best classification results on ABIDE1 dataset for different parcellations.}
\label{table:results}
\end{table}


==> tables/table1_single.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{2.5cm}lll|}
\hline
                               & \multicolumn{1}{c}{\small 1-voxel} & \multicolumn{2}{c|}{\small Multi-voxel}                 \\
                               & \multicolumn{1}{c}{\textbf{pCor}}       & \multicolumn{1}{c}{\textbf{dCor}} & \multicolumn{1}{c|}{\textbf{WFC}} \\ \hline \hline
\multicolumn{1}{|l|}{Caltech}  &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{KKI}      &~\textbf{00.0$\pm$0.0}           &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{Leuven}   &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{MaxMun}   &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{NYU}      &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{OHSU}     &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{Olin}     &~\textbf{00.0$\pm$0.0}           &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{Pitt}     &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{SBL}      &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{SDSU}     &~\textbf{00.0$\pm$0.0}           &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{Stanford} &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{Trinity}  &~\textbf{00.0$\pm$0.0}           &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{UCLA}     &~\textbf{00.0$\pm$0.0}           &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{UM}       &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{USM}      &~00.0$\pm$0.0                    &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\
\multicolumn{1}{|l|}{Yale}     &~\textbf{00.0$\pm$0.0}           &~00.0$\pm$0.0               &~00.0$\pm$0.0~                \\ \hline
\end{tabular}
\caption{Wasserstein functional connectivity. Best classification results on ABIDE1 dataset for different sites.}
\label{table:results}
\end{table}


==> tables/table2.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{|p{2.7cm}p{2.6cm}p{1.5cm}p{2.4cm}p{2.4cm}|}
\hline
 \textbf{Atlas, \#ROIs} & \textbf{Mode}  & \textbf{Site} & \textbf{Tangent} \cite{Dadi2019} & \textbf{Mean shift} \\ \hline \hline
 
 \multirow{6}{*}{MSDL \cite{Varoquaux2011}, $49$}
% & All sites        &       &        &  \\
 & Ind. site        & TT1   &        &  \\
 &                  & TT2   & 0.7235 & \textbf{0.7955} \\
 &                  & BG    & 0.7158 & \textbf{0.7814} \\
 & Leave-site-out   & TT1   & 0.7010 & \textbf{0.7707} \\
 &                  & TT2   &        &  \\
 &                  & BG    &        &  \\ \hline \hline
 
 \multirow{6}{*}{AAL \cite{Tzourio2002}, $116$}
% & All sites        &       & 0.0000 & 0.0000 \\
 & Ind. site        & TT1   & 0.7937 & \textbf{0.8219} \\
 &                  & TT2   & 0.8062 & \textbf{0.8119} \\
 &                  & BG    & 0.8043 & \textbf{0.8152} \\
 & Leave-site-out   & TT1   & 0.7719 & \textbf{0.7974} \\
 &                  & TT2   & 0.7782 & \textbf{0.8285} \\
 &                  & BG    &  & \\ \hline \hline 
 
 \multirow{6}{*}{BASC \cite{Bellec2010}, $197$}
% & All sites        &       & 0.0000 & 0.0000 \\
 & Ind. site        & TT1   &  &  \\
 &                  & TT2   & \textbf{0.8355} & 0.8186 \\
 &                  & BG    & 0.8734 & \textbf{0.8814} \\
 & Leave-site-out   & TT1   &  &  \\
 &                  & TT2   &  &  \\
 &                  & BG    &  &  \\ \hline
\end{tabular}

\vspace{0.33em}
\caption{ROC AUC metric for the binary classification problem is reported for $5$-fold cross-validation averaged over $10$ runs.}
\label{tab:my-table}
\end{table*}
